Compositional design for time-varying and nonlinear coordination

This work addresses the design of multi-agent coordination through high-order consensus protocols. While first-order consensus strategies are well-studied -- with known robustness to uncertainties such as time delays, time-varying weights, and nonlinearities like saturations -- the theoretical guarantees for high-order consensus are comparatively limited. We propose a compositional control framework that generates high-order consensus protocols by serially connecting stable first-order consensus operators. Under mild assumptions, we establish that the resulting high-order system inherits stability properties from its components. The proposed design is versatile and supports a wide range of real-world constraints. This is demonstrated through applications inspired by vehicular formation control, including protocols with time-varying weights, bounded time-varying delays, and saturated inputs. We derive theoretical guarantees for these settings using the proposed compositional approach and demonstrate the advantages gained compared to conventional protocols in simulations.

==> articlefiles/oldfiles/CaseStudy.tex <==
Here, we consider a network of double-integrator systems
\begin{equation}
    \ddot{x}_i=u_i(x).
    \label{eq:double_integrators}
\end{equation}
When restricted to only using relative feedback, a natural choice of controller is a second-order consensus system; both conventional and serial consensus can work. However, independent of the choice of second-order consensus system, the closed loop cannot reject load disturbances without a stationary error. This can be seen by the fixed point conditions $L_0x=w\neq 0$ and $L_2L_1x=w\neq 0 \implies L_1x \neq 0$ respectively. For measurable disturbances and with perfectly known dynamics, it is possible to design a feedforward term to reject any disturbance. Alternatively, an integral feedback term can be incorporated to handle unmeasured disturbances. In \cite{TEGLING2023}, it was shown that distributed third-order conventional consensus may lose stability as more agents are added to the network. On the other hand, serial consensus is stable for any order \cite{Hansson2023CDC}. We will, therefore, focus on the third-order serial consensus to handle potential load disturbances in the system. Following the serial-consensus design, the following feedback law can be utilized
\begin{equation}
\begin{aligned}
    u(x)&=-\underbrace{(p_1+p_2+p_3)}_{a_\mathrm{v}} L\dot{x}\\
    -&\underbrace{(p_1p_2+p_1p_3+p_2p_3)}_{a_\mathrm{p}}L^2(x-d)-\underbrace{(p_1p_2p_3)}_{a_{\mathrm{I}}}Lz\\
    \dot z&=L^2(x-d).
\end{aligned}
\label{eq:serial_controller}
\end{equation}
The closed-loop system can then be analyzed in terms of the states $\dot{x}$, $L(x-d)$, and $z$ which has the form
\begin{equation}
\bmat{\dot{z}\\L\dot{(x-d)}\!\!\\ \ddot x}\!\!=\!\!
\bmat{ 0&L&0\\
       0&0&L\\
       \!-a_{\mathrm{I}}L&\!\!\!-{a_\mathrm{p}}L&\!\!\!-{a_\mathrm{v}}L}
   \!\!\bmat{z\\L(x-d)\\ \dot x}\!\!+\!\!\bmat{0\\ 0\\w}\!\!.
\label{eq:3rdOrderSerial}   
\end{equation}
This is of the same form as described in Theorem~\ref{thrm:nth_serial_performance}, so it will also exhibit scalable performance in terms of the transient deviation from any initial condition.

\subsection{Disturbance rejection}
Since only relative feedback is used, it is impossible to guarantee that any load disturbance can be rejected; in fact, only the disturbances in the image of $L$ will be observable. For instance, the response to the constant disturbance $w=\mathbf{1}$ with all states starting at the origin will have the response
$$\dfrac{1^T\dot{x}(t)}{N}=t.$$
But when the disturbance lies in the image, or if we only consider the relative states, the disturbance will be asymptotically rejected as per the following theorem.
\begin{theorem}\label{thrm:3order_dserial}
    The third-order serial consensus system \eqref{eq:3rdOrderSerial} with $w(t)=Lw_0$, where $w_0$ is constant, and where the graph underlying $L$ contains a directed spanning tree,  will achieve $L(x-d)\to 0$ and $L\dot{x}\to 0$ as $t\to \infty$ and satisfy
    $$\sup_{t\geq 0}\|\xi(t)\|_\infty\leq \alpha_\xi(p)\|\xi(0)\|_\infty +\alpha_w(p)\|w_0\|_\infty,$$
    with the bounds quantified by the constants $\alpha_w(p) =\frac{2}{p_1p_2p_3}\|S_1\|_\infty\|S_1^{-1}[1,0,0]^\top\!\|_\infty\!$ and $\alpha_\xi(p)=\|S_2\|_\infty\|S_2^{-1}\|_\infty$ where $S_1,S_2$ are any matrices that diagonalize $A$.
\end{theorem}
\vspace{1ex}
The proof is found in the appendix.
This theorem shows that the PI-controlled vehicle formation will have scalable performance, and load disturbances will not lead to any stationary error. We remark that $\alpha_w$ and $\alpha_\xi$ can be optimized by following the procedure outlined in Lemma~\ref{lem:minnorm}.


==> articlefiles/oldfiles/ConsensusSystems.tex <==
\section{First-order consensus results}

\subsection{Time-varying coefficients}
Here we will consider the following consensus protocol 
\begin{equation}
    \dot{\xi}=-L(t)\xi(t)+\ur 
    \label{eq:timeconsensus}
\end{equation}
where $L(t)$ is for every time $t$ a graph Laplacian, thus satisfying $L(t)\mathbf{1}=0$. Following the notation of (L Moreau), if there exists a time $\infty>T> 0$, a node $k$ reachable from every other node through a path with a minimum degree $a_{\min}>0$. Let the integrated graph Laplacian be
$$A(t)=\int_t^{t+T}L(\tau)\mathrm{d}\tau$$
If $k$ is reachable through a path with a minimum degree $a_{\min}$ and maximum degree $a_{\max}$ from every other node $j\neq k$ in the graph underlying $A(t)$, for all $t$, then the system will asymptotically reach consensus.

A few simple examples of how the time-varying capabilities can be utilized in the serial consensus can be considered as follows. Perhaps the simplest is the second-order serial consensus system when $\Lc_2=L_2(t)$ and $Lc_1(t,x)=L_1(t)x$ where the closed loop becomes
$$\ddot{x}=(-L_2(t)-L_1(t))\dot{x}-(L_2(t)L_1(t)+\dot{L}_1(t))x+u_\mathrm{ref}(t).$$
From this system we can see that changes of $L_2(t)$ can be made quite arbitrarily while for $L_1(t)$ its derivative must also be taken into account as it varies in time. It's worth noting that a localized $L_1(t)$ implies the same locality of $\dot{L}_1(t)$, so from the perspective of having a localized controller, no further restrictions are added.


\subsection{Input time-varying time delays}

Here we will consider two types of time delays. First, we consider the case of input delay. This may occur due to the time of sensing, or perhaps local message passes. The corresponding first-order system that represent this scenario is
$$\dot{x}=-S_\tau Lx(t)+\ur(t),$$
where $S_\tau y(t)=\mathrm{vec}(y_1(t-\tau_1(t),\dots,y_n(t-\tau_n(t))$ where $\tau_k$ is a bounded time-varying delay function. For this type of time delay, there exists sufficient results which guarantee stability for sufficiently small delays. For the implementation of serial consensus its reasonable to assume that an implementation delay would occur if message passing is implemented. This can be modeled and avoided through either including delay operator in the first or second operator.

\subsection{Alternative time delay}

An alternative and more scalably robust time-delay is the following
$$\dot{\xi}_i=-M(t)xi_i(t)+\ur+\sum_{j\in \mathcal{N}_i} w_{i,j}(t)\xi_j(t-\tau_{i,j}(t))$$
This system is globally exponentially stable, as long as the time-delays have a bound, and as long as the graph Laplacian $L(t)=-M(t)+W$ is a graph Laplacian with an underlying graph that is over time sufficiently connected, $M$ is a non-negative diagonal matrix, and $W$ a non-negative matrix as has been established in \cite{Moreau2004stabconsensus, jour:Lu2017consensusdelays}.

When restricted to only use relative feedback the following equivalent version of the above can be used:

$$\dot{x}_i(t)=\!\!\sum_{j\in \mathcal{N}_i} \!\!w_{i,j}(t) \left(S_{\tau_{i,j}}x_i(t)-x_i(t)+S_{\tau_{i,j}}(x_i(t)-x_j(t))\right)$$
where, if all measurements are synchronized this simplifies to
$$\dot{x}=-P(x-S_\tau x)+\ur+\sum_{j\in \mathcal{N}_i}- S_\tau Lx$$
Here, the simple criterion for stability is that $p_i\geq \sum_{j\in \mathcal{N}_i}w_{i,j}$.

One interesting application of this control law utilizing this property is when incorporating a GPS signal for vehicle platooning. Some considerations of using such a signal is 1) the signal may be noisy, and there is a delay that also may depend on time to sample losses. The uncertainties calls for the use of a small gain. The upside, is that short convergence times can be guaranteed, since the GPS signal essentially introduces absolute feedback. Let 
$\Lc_2(t,x)=-Lx(t)-P_\mathrm{GPS}(x-S_\tau x+S_\tau (x-x_\mathrm{ref})$ and $\Lc_1(x)=Lx$. In this setup, the joint controller is 
$$u(x)=\Lc_2(Lx+\dot{x})+L\dot{x}=L^2x+2L\dot{x}+P_\mathrm{GPS}(Lx+\dot{x}-S_\tau\dot{x}_\mathrm{ref})$$
Here, all vehicle velocity sensors might not be perfectly synced, to get rid of this issue, the vehicles can instead utilize the following formulation: $\dot{x}-S_\tau x_\mathrm{ref}=\dot{x}-S_\tau \dot{x}+S_\tau (\dot{x}-\dot{x}_\mathrm{ref})$.


\subsection{Saturated signals}
As a final example of a consensus protocol that can be used in the serial consensus formulation we consider the scenario where the control signal has a saturation, which corresponds to the following system:
$$\dot{x}=-\mathrm{sat}(Lx)+u_\mathrm{ref}.$$
Where $\mathrm{sat}(\cdot)$ denotes the elementwise saturation function. A corresponding second-order consensus protocol would then have the following controller:
$$u(x)=\mathrm{sat}\left(L^2x+L\dot{x}\right)+L\dot{x}$$

(It's not completely obvious what benefit is gained by using the saturation here since the linear protocol is string stable and the control signal will thusly have a bounded signal.

==> articlefiles/oldfiles/ConsensusSystemsFinal.tex <==
\section{First-order consensus results}
Here we will recall some known results on continuous-time consensus protocols and relate them to Theorem~\ref{thrm:nonlinear_serial}. 
\subsection{Time-varying consensus}
A common property of real physical systems is that the gain might vary over time, and the assumption of true time-invariant linearity might be an over-restrictive requirement. Instead, consider the time-varying consensus protocol
$$\dot{x}=-L(t)x+\ur.$$
In \cite{Moreau2004stabconsensus}, a simple condition for the time-varying consensus to reach a consensus is provided; consensus will be reached if there exists a $0<T<\infty$, such that the following matrix
$$M(t)=\int_t^{t+T} L(\tau)\mathrm{d}\tau$$
is sufficiently connected for every $t\geq 0$. Formally, there needs to exist an agent $k$ which has a path to any other agent $j$ with a path that consists of edges with a uniform minimum edge weight. As a simple example, any graph time-varying graph Laplacian that can be expressed as $L(t)=L_0 +L_1(t)$ where $L_0$ contains a spanning tree and $L_1(t)$ is a graph Laplacian for any time $t$ fulfills this requirement.

\subsection{Actuation delay systems}
A common occurrence in controlled systems are time-delays, one such can appear as the consequence of the inherent delay between sensing and actuation. To write this compactly we introduce a delay operator:
$$\mc{D}_\tau x(t)=\bmat{x_1(t-\tau_1(t))\\ x_2(t-\tau_2(t))\\ \vdots \\ x_N(t-\tau_N(t))}.$$
Now the actuation delayed consensus system can be described as
$$\dot{x}=-\mc{D}_\tau Lx(t)+ \ur(t)$$
Here, stability can be guaranteed through (theorem from survey) if the eigenvalues ...

\subsection{Off-diagonal delays}
Depending on the limitation of the consensus protocol, larger delays is permitted if the delays only enter through the off-diagonal elements, that is, if the dynamics can be described as

$$\dot{x}_i=-d_{ii}(t) x_i(t)+\ur+\sum_{j\in \mc{N}_i} w_{i,j}(t)x_j(t-\tau_{i,j}(t))$$
As long as $L(t)=D(t)-W(t)$ satisfy the condition for being a sufficiently connected Laplacian and there exists a finite $\tau_\mathrm{max}\geq \tau_{i,j}(t)$ for all $t$, then this delayed consensus system will converge to a consensus \cite{Moreau2004stabconsensus,jour:Lu2017consensusdelays}.

\subsection{Saturated inputs}
As a final example of a stable consensus protocol, consider the consensus system where the control effort is saturated:
$$\dot{x}_i=\ur^i-\sat\left( d_ix_i(t) -\sum_{j\in \mc{N}_i}w_{i,j} x_j(t) \right)$$
This system will asymptotically achieve consensus if $L\ur \to 0$. 
\begin{proof}
    Since the dynamics are described by an $\Lc(x,t)$ that is Lipschitz in $x$ and piecewise continuous in $t$, it follows that a solution exists and is unique for all time $t\geq 0$. So WLOG, $\|L\ur\|< 1$ can be assumed and an arbitrary initial condition $x_0$.
\end{proof}

To see this, conside




==> articlefiles/oldfiles/Introduction.tex <==
\emma{For Introduction: \textbf{1)} more references. \textbf{2)} Put in the context of other compositional/iterconnection results. why it is relevant to infer stability and performance of a system composed of simpler systems (this is central in control!). What apporoaches exist: SGT, passivity, contraction... \textbf{3)} Relation to Arcak's work (call it `ìnfluential''). What do we do that he didn't? \textbf{4)} why are we revisiting this old problem? (references are 10+ ys old). I think you can point to scale fragility result and the question of scalability.  \textbf{5)} Say something about the cost of doing serial consensus, ie more connections/communication.}

Consensus protocols have been widely studied as a foundational tool for multi-agent coordination. Originating in models of opinion dynamics~\cite{degroot1974reaching}, these protocols describe how agents in a network align their states through local interactions. In the continuous-time setting, agents adjust their dynamics in proportion to disagreements with neighbors, leading to global convergence under suitable connectivity conditions. This framework has since been applied to multi-agent coordination control problems with some seminal works by \cite{jour:Jadbabaie2003,jour:FaxMurray2004, olfati2004consensusdelays}.

% The problem of achieving consensus is a vastly studied topic. Some pioneering works were made to model opinion dynamics \cite{degroot1974reaching}. In this setting, a weighted average of each individual's friends' opinions is taken, guiding the opinion evolution. Given sufficient connectivity, this process eventually leads to the networked system reaching a consensus. A corresponding continuous-time result exists; here, the rate of change is updated proportionally to the local deviations, and through these simple interactions, the agents eventually reach a consensus. This idea has been applied to the problem of multi-agent coordination with some seminal works by \cite{jour:Jadbabaie2003,jour:FaxMurray2004, olfati2004consensusdelays}.

\emma{Not sure I agree that high-order consensus is only a generalization of first-order. Second-order is very natural to pose for physical agents with mass}


The many works that have considered the generalization of consensus protocols to achieve high-order consensus protocols are relevant to this work. Perhaps the simplest one is the linear protocol, which utilizes relative measurements of positions, velocities, accelerations, and so on. Following the notation of \cite{jour:Ren2007}, the closed-loop system dynamics are
\[
x^{(n)}=-r_{(n-1)}Lx^{(n-1)}-\cdots-r_{(1)}L\dot{x}-r_{(0)}Lx.
\]
Given a sufficiently connected graph Laplacian $L$ together with properly tuned constants $r_k$, this system will manage to coordinate the positions $x$, the velocities $\dot{x}$, all the way up to $x^{(n-1)}$, which represent the $(n-1)$th derivative. What constitutes properly chosen weights depends on the order of the system. For the first-order case, any positive scaling is sufficient. In the second-order case, a real spectrum of $L$ (e.g., the Laplacian is symmetric or triangular) with positive weights $r_0$, $r_1$ is sufficient. For Laplacians with a complex spectrum, more caution is needed to avoid instability, which might occur in the case of large directed cycles \cite{jour:Studli2017}. For high-order $(n\geq 3)$, there is no choice of weights $r_k$ that universally work for any graph Laplacian, and instead, the weights $r_k$ must be chosen based on the spectrum of the $L$ to ensure the system's stability \cite{jour:TEGLING2023}.

Some works have considered the problem of high-order coordination (see survey ). By far, the most well-studied is the second-order case.


% (old ref on this). The studies of systems that eventually reach consensus have widespread applications---power systems ( XX), multi-agent coordination, distributed optimization and opinion dynamics. Other systems often modeled through consensus interactions include flocking behavior, spontaneous synchronization, and partial differential equations (like advection, diffusion, and the beam equation).

% Of particular interest for this study are the works on multi-agent coordination pioneered by the works (Fax Murray, Moreau, ...). Listing all the works on multi-agent coordination and the contributions thereof would be an arduous task, excellently carried out by (multi-agent coordination summary). 


This work presents a framework for combining many works on first-order consensus to achieve high-order consensus. The main idea originates from our works on high-order serial consensus \cite{jour:hansson2023scalable,jour:hansson2024lcss}. Serial consensus can be seen as a design method to achieve a desired closed-loop system, reminiscent of pole placement and the famous Youla-Kucera parametrization. In a nutshell, we search for the controller that leads to a desired closed-loop system. In the earlier-mentioned works, we have suggested the serial-consensus system, which in the second-order case is
$$\ddot{x}=-(p_1+p_2)L\dot{x}-p_1p_2L^2x+u_\mathrm{ref}(t).$$
This system can be robust while enjoying strong properties, such as string stability \cite{jour:hansson2025tcns}. 
 

While the simplicity of the serial consensus protocol makes it desirable, the lack of a methodology for handling potential nonlinearities and more general setups, such as sampled control, limits its practical applicability. A real-world implementation was tested in \cite{Oorschot2024}, demonstrating good performance despite the introduced uncertainties. In this work, we show that serial consensus can be extended to include many first-order consensus protocols that are not necessarily restricted to linear ones. We propose the controller that corresponds to the following closed-loop system 
$$\left((\dt+\Lc_n)\circ \cdots \circ (\dt+\Lc_2)\circ (\dt+\Lc_1)\right)(x)=u_\mathrm{ref}. $$
Our main result essentially shows that as long as each first-order system 
$$\dot{x}=-\Lc_k(t,x) +u_\mathrm{ref}$$
would reach a consensus, then the composition will reach an $n$\ts{th}-order consensus, thus achieving simultaneous synchronization in its $n$ first derivatives. The generality of this result allows us to show that consensus can be guaranteed under the presence of time-varying weights, time-varying delays, and various nonlinearities such as saturations. A special case of the permitted time-varying delays is the sampled system, which allows us to prove the results of hybrid consensus systems. 

The paper is outlined as follows: First, we will introduce some necessary mathematical preliminaries. Then, we'll show and prove our main result. We'll devote a section introducing some established first-order consensus results, followed by examples illustrating many interesting multi-agent coordination results. Then, we will discuss directions for future work and provide our conclusions.

\subsection{Mathematical Preliminaries}
\paragraph*{Graph Theory}
We represent a directed graph as \( \mathcal{G} = (\mathcal{V}, \mathcal{E}) \), where \( \mathcal{V} = \{1, \dots, N\} \) is the set of nodes, and \( \mathcal{E} \subset \mathcal{V} \times \mathcal{V} \) is the set of edges. The graph is associated with a weighted adjacency matrix \( W \in \mathbb{R}^{N \times N} \), where \( W_{i,j} > 0 \) if and only if \( (j, i) \in \mathcal{E} \), i.e., agent \( j \) influences agent \( i \).

The corresponding graph Laplacian is defined as
\[
L = D - W,
\]
where \( D \) is the diagonal degree matrix with \( D_{i,i} = \sum_{j=1}^N W_{i,j} \). The graph Laplacian \( L \) has zero row sum and encodes the relative feedback structure of the network.

A graph is said to contain a \emph{directed spanning tree} if there exists a node \( k \in \mathcal{V} \) such that all other nodes \( j \in \mathcal{V} \setminus \{k\} \) are reachable via a directed path from \( k \). If this condition holds, the Laplacian \( L \) has a simple zero eigenvalue, and all other eigenvalues have strictly positive real parts.

We also make use of \emph{\( \delta \)-graphs} as defined in~\cite{Moreau2004stabconsensus}. Given a threshold \( \delta > 0 \), the \( \delta \)-graph associated with \( W \) is a subgraph where an edge \( (j, i) \) is retained if and only if \( W_{i,j} \geq \delta \).

% \subsubsection{Graph theory}
% We denote a graph as $\mathcal{G}(\mathcal{V},\mathcal{E})$ with $N=|\mathcal{V}|$ vertices and $\mathcal{E}\subset \mathcal{V}\times \mathcal{V}$ edges. The graph can also be defined with the adjacency matrix $W$, where $W_{i,j}>0 \iff(j,i)\in \mathcal{E}.$ Associated with an adjacency matrix, the graph Laplacian can be constructed as 
% $$L=D-W$$
% where $D$ is a diagonal matrix with its $i$\ts{th} element defined as $D_{ii}=\sum_{j=1}^N W_{ij}$. 

% A graph is said to contain a directed spanning tree if a node $k\in \mc{V}$ exists such that every other node $j \in \mc{V}\setminus k$ is reachable through a path originating from $k$. If a graph contains a directed spanning tree, its graph Laplacian will have a unique zero eigenvalue, and all other eigenvalues will have strictly positive real parts. We will also use $\delta$-graphs, following the definition in \cite{Moreau2004stabconsensus}. These are directed graphs with edge weight $w_{i,j}>0\iff w_{i,j}\geq \delta$, and from any graph Laplacian, we may construct the corresponding $\delta$-graph by removing the edges with weights below the $\delta$ threshold.
\paragraph*{Norms and Notation}
We denote vector and matrix norms using \( \|\cdot\| \). For vectors \( x \in \mathbb{C}^N \), we use the \( \infty \)-norm
\[
\|x\|_\infty = \max_i |x_i|,
\]
and for matrices \( C \in \mathbb{C}^{N \times N} \), the induced matrix norm
\[
\|C\|_\infty = \max_i \sum_j |C_{ij}|.
\]
Seminorms are denoted \( \vertiii{\cdot} \), following the notation in~\cite{bullo2024-CTDS}. When the context is clear, we drop explicit time-dependence \( x(t) \). We write \( \dtk{j} x = x^{(j)} \) for the \( j \)\ts{th} time derivative, and use \( \partial_t F(x,t) \) for partial derivatives.

Function composition is written \( (f \circ g)(x) = f(g(x)) \). When composing time-varying functions, we use the convention
\[
(\Lc_2 \circ \Lc_1)(x) := \Lc_2(\Lc_1(x,t), t).
\]

% Throughout this article, we will use standard notation for norms, where $\|\cdot\|$ denotes any unspecified norm. With $\|x\|_\infty=\max_i |x_i|$ when $x\in \mathbb{C}^N$, and we use the same notation for the corresponding induced matrix norm $\|C\|_\infty=\max_i \sum_j |C_{i,j}|$. By $\vertiii{\cdot}$, we denote seminorms following the notation in \cite{bullo2024-CTDS}. Explicit time-dependence will be dropped $x(t)$ when the context is clear. $\dtk{j}x=x^{(j)}$ will be used to denote the $j\ts{th}$ time derivative and $\partial_t F(x,t)$ for the partial derivative. Function compositions will be denoted $(f\circ g)(x)=f(g(x))$ and when composing time-varying function we will sometimes use $(\Lc_2 \circ \Lc_1)(x)=\Lc_2(\Lc_1(x,t),t)$.

\subsection{Consensus}
A central concept in this work is that of \emph{consensus} among agents in a network.

\begin{definition}[Consensus]\label{def:consensus}
Let \( x(t) \in \mathbb{R}^N \) be the state of a multi-agent system governed by
\[
\dot{x} = f(x,t).
\]
The system is said to achieve \emph{consensus} if
\[
\lim_{t \to \infty} |x_i(t) - x_j(t)| = 0, \quad \text{for all } i \neq j.
\]
\end{definition}

A classical example that manages to achieve consensus is 
\[
\dot{x} = -Lx,
\]
where \( L \) is a graph Laplacian where the underlying graph contains a directed spanning tree.

In high-order coordination problems, it is often desirable to synchronize the positions and higher-order derivatives such as velocities and accelerations. This motivates the following generalization:

\begin{definition}[\( n\ts{th} \)-Order Consensus]
Let \( x(t) \in \mathbb{R}^N \) evolve according to
\[
\frac{\mathrm{d}^n x}{\mathrm{d}t^n} = f(x,t).
\]
The system is said to achieve \( n\ts{th} \)-order consensus if
\[
\lim_{t \to \infty} |x_i^{(k)}(t) - x_j^{(k)}(t)| = 0, \quad \text{for all } i \neq j \text{ and } k = 0, \dots, n-1.
\]
\end{definition}
This definition captures the idea that all agents eventually align in their positions and higher-order dynamics, like velocities and accelerations.


==> articlefiles/oldfiles/MainResultFinal.tex <==
\section{Main Results}


Our main result concerns the stability of the compositional coordination scheme and is summarized as follows:
\begin{theorem}\label{thrm:nonlinear_serial}
Consider the compositional consensus system \eqref{eq:nonlinear_serial} where $\Lc_n$ and $\ur$ satisfy Assumption~\ref{ass:stab_cons1} and where $\Lc_k$ for $k\neq n$ satisfy Assumption~\ref{ass:stab_cons2}--\ref{ass:existandunique}. Then, the solution $x(t)$ will achieve an $n\ts{th}$-order consensus.
\end{theorem}\vspace{0.5em}

Essentially, this theorem establishes that any composition of effective first-order consensus protocol can be combined in a structured way to construct a high-order consensus protocol.

\begin{proof}
    First we transform the system to an equivalent ODE formulation:
    $$
    \bmat{\dot{\xi}_1\\ \vdots \\\dot{\xi}_n}=\bmat{ \Lc_1(\xi_1,t)+\xi_2\\ \vdots \\ \Lc_n(\xi_n,t)+u_\mathrm{ref}},
    $$
    where $x=\xi_1$, $x^{(k)}=\xi_{k+1}-\Lc_k(\xi_k,t)$. Next, we show that the asymptotic consensus of the states $\xi_k$ is equivalent to $x$ achieving $n$\ts{th}-order consensus. In the forward direction we have $\|\xi_k-\mathbf{1}\alpha_k(t)\|\to 0$, this implies that
    $$x^{(k)}(t)-\mathbf{1}\alpha_{k+1}(t)=\xi_{k+1}(t)-\mathbf{1}\alpha_{k+1}(t)-\Lc_k(\xi_k-\mathbf{1}\alpha_k(t),t)$$
    Where we used that $\Lc_k(x+\mathbf{1}y,t)=\Lc_k(x,t)$. Utilizing that $\Lc_k$ is Lipschitz in $x$ and the triangle inequality shows
    $$\|x^{(k)}-\mathbf{1}\alpha_{k+1}\|\leq \|\xi_{k+1}-\mathbf{1}\alpha_{k+1}\|+C_k\|\xi_{k}-\mathbf{1}\alpha_{k}\|, $$
    which shows that $\lim_{t\to\infty}\|x^{(k)}-\mathbf{1}\alpha_{k+1}\|=0.$ The same also holds true for $\|x-\mathbf{1}\alpha_1\|$. In the other direction we can use induction. The base case that $\|x-\1\beta_0\|\to 0 \implies \|\xi_1-\1\beta_0\|\to 0$ is simple. For the rest, we show that if $\|x^{(k)}-\1\beta_k\|\to 0$ and $\|\xi_k(t)-\alpha_k(t)\|$, then there is $\alpha_{k+1}(t)$ such that $\|\xi_{k+1}(t)-\1 \alpha_{k+1}(t)\|\to 0$. This implication holds, since 
    $$\xi_{k+1}-\1\beta_k=x^{(k)}-\1\beta_k+\Lc_k(\xi_k-\1\alpha_k,t),$$
    which shows that $\|\xi_{k+1}-\1\beta_{k+1}\|\to 0$, due to $\Lc_k$ being Lipschitz, and that the induction is only performed for a finite number of steps.

    
    We will now show, through induction, that $\|\xi_{k+1}-\1\alpha_{k+1}\|\to0\implies \|\xi_k-\1\alpha_k\|\to 1$. Here, we let the base case be $\xi_{n+1}=\ur$, with $\alpha_{n+1}=u_0(t)$, which exists by assumption. We have
    $$\dfrac{\mathrm{d}}{\mathrm{d}t}\left(\xi_k-\1\tilde{\alpha}_k\right)=-\Lc_k(\xi_k-\1\tilde{\alpha}_k,t)+\xi_{k+1}-\1\alpha_{k+1}$$
    where $\tilde{\alpha}_{k}=\int^t_0 \alpha_{k+1}(\tau)\mathrm{d}\tau$. By Assumption~\ref{ass:stab_cons}, we can conclude that that there is $a_k$ such that $\|\xi_k-\1(\tilde{\alpha}_k+a_k)\|\to 0$, letting $\alpha_k=\tilde{\alpha}_k+a_k$ concludes the induction step. By the equivalence of consensus it follows that $x$ achieves $n$\ts{th}-order consensus.
\end{proof}


==> articlefiles/oldfiles/MainResults.tex <==
\section{Main Results}
% \subsection{notation}
% We denote function composition by $(g\circ h)(x)=g(h(x)).$

% We denote weakly contracting systems as
% $\dot{x}=-F(x,t)$
% where for every pair of solutions $x_1,x_2$ the following holds true:
% $$\|x_2-x_1\|\leq \|x_2(0)-x_1(0)\| $$

% \subsection{result}
% Here, we characterize how weakly contracting systems can be interconnected.
% \begin{ass}[Stable consensus]\label{ass:stab_cons}
%     The function $\Lc_k(x,t)$ are chosen such that the following system satisfies
%     $$\dot{x}=-\Lc_k(x,t)+\ur$$
%     $\|\ur(t)\|\to 0\implies \exists a_k(t) \text{ s.t. } \|x(t)-\1a_k(t)\|\to 0$.
% \end{ass}

% \begin{ass}[Consensus invariance]\label{ass:invariance} $\Lc_k(x,t)$ satisfy
%     $$\Lc_k(x+a \1,t)=\Lc_k(x,t),\;\forall a\in \R, x\in \RN.$$
% \end{ass}

% \begin{ass}[Existance and uniqueness] Potentially, we should assume that each $\Lc_k(x,t)$ is Lipschitz in $x$ and piecewise-continuous in $t$, with at most countable discontinuities.
% \end{ass}

% \begin{theorem}
% Let all $\Lc_k$ satisfy Assumption~\ref{ass:stab_cons} and \ref{ass:invariance}. The following system
% \begin{equation}
% \label{eq:nonlinear_serial}
%     \left((\frac{\mathrm{d}}{\mathrm{d}t}+\Lc_n)\circ \cdots \circ (\frac{\mathrm{d}}{\mathrm{d}t}+\Lc_1) \right)(x,t)=\ur
% \end{equation}
% will achieve $n\ts{th}$-order consensus if and only if there exists $u_0(t)$ s.t. $\|\ur(t)-\1 u_0(t)\|\to 0.$    
% \end{theorem}
% \begin{proof}
%     We start by identifying a convenient state-space representation of \eqref{eq:nonlinear_serial}:
%     \[
%     \bmat{\dot{\xi}_1\\ \vdots\\ \dot{\xi}_n}=\bmat{-\mathcal{L}_1(\xi_1,t)+\xi_2\\\vdots\\ -\mathcal{L}_n(\xi_n,t)+u_\mathrm{ref}}
%     \]
%     Where $x=\xi_1$, $x^{(k)}=\xi_{k+1}-\mathcal{L}_{k}(\xi_k,t),$
%     Next, we show that the asymptotic consensus of the states $\xi_k$ is equivalent to $x$ achieving $n$\ts{th}-order consensus. In the forward direction we have $\|\xi_k-\mathbf{1}\alpha_k(t)\|\to 0$, this implies that
%     $$x^{(k)}(t)-\mathbf{1}\alpha_{k+1}(t)=\xi_{k+1}(t)-\mathbf{1}\alpha_{k+1}(t)-\Lc_k(\xi_k-\mathbf{1}\alpha_k(t),t)$$
%     Where we used that $\Lc_k(x+\mathbf{1}y,t)=\Lc_k(x,t)$. Utilizing that $\Lc_k$ is Lipschitz in $x$ and the triangle inequality shows
%     $$\|x^{(k)}-\mathbf{1}\alpha_{k+1}\|\leq \|\xi_{k+1}-\mathbf{1}\alpha_{k+1}\|+C_k\|\xi_{k}-\mathbf{1}\alpha_{k}\|, $$
%     which shows that $\lim_{t\to\infty}\|x^{(k)}-\mathbf{1}\alpha_{k+1}\|=0.$ The same also holds true for $\|x-\mathbf{1}\alpha_1\|$. In the other direction we can use induction. The base case that $\|x-\1\beta_0\|\to 0 \implies \|\xi_1-\1\beta_0\|\to 0$ is simple. For the rest, we show that if $\|x^{(k)}-\1\beta_k\|\to 0$ and $\|\xi_k(t)-\alpha_k(t)\|$, then there is $\alpha_{k+1}(t)$ such that $\|\xi_{k+1}(t)-\1 \alpha_{k+1}(t)\|\to 0$. This implication holds, since 
%     $$\xi_{k+1}-\1\beta_k=x^{(k)}-\1\beta_k+\Lc_k(\xi_k-\1\alpha_k,t),$$
%     which shows that $\|\xi_{k+1}-\1\beta_{k+1}\|\to 0$, due to $\Lc_k$ being Lipschitz, and that the induction is only performed for a finite number of steps.

%     With the equivalence established, we now show that there exist constants $\alpha_k$ such that $\|\xi_{k}-\1\alpha_k\|\to 0$. But first, we consider the case where there is no $u_0(t)$ such that $u_\mathrm{ref}-\1u_0(t)\not\to 0$. By way of contradiction, assume that $\|\xi_k-\1\alpha_k\|\to 0$ for some $\alpha_k$. Then, in particular, 
%     \begin{multline*}
%         C_n\|\xi_n-\1\alpha_n\|\geq\|\Lc(\xi_n-\1\alpha_n,t)\|=\|\ur-\dot{\xi}_n\|\\
%         \geq \inf_{u_0}\|\ur-\1u_o(t)\|-\|\frac{\mathrm{d}}{\mathrm{d}t}(\xi_n-\1\alpha_n)\|
%     \end{multline*}
%     \textbf{Is the following a consequence, or do I need another assumption?} Now, due to X, $\xi_n-\1\alpha_n$ and its derivative will converge to $0$, which contradicts that $u_\mathrm{ref}-\1u_0(t)$ does not converge to $0$. Since the consensus of $\xi_k$ is equivalent to the high-order consensus of $x$, this shows that there has to exist a $u_0$ such that $u_\mathrm{ref}$ achieves consensus for $n$\ts{th}-order consensus to be achieved.
    
%     Under this assumption we will now show, through induction, that $\|\xi_{k+1}-\1\alpha_{k+1}\|\to0\implies \|\xi_k-\1\alpha_k\|\to 1$. Here, we let the base case be $\xi_{n+1}=\ur$, with $\alpha_{n+1}=u_0(t)$, which exists by assumption. We have
%     $$\dfrac{\mathrm{d}}{\mathrm{d}t}\left(\xi_k-\1\tilde{\alpha}_k\right)=-\Lc_k(\xi_k-\1\tilde{\alpha}_k,t)+\xi_{k+1}-\1\alpha_{k+1}$$
%     where $\tilde{\alpha}_{k}=\int^t_0 \alpha_{k+1}(\tau)\mathrm{d}\tau$. By Assumption~\ref{ass:stab_cons}, we can conclude that that there is $a_k$ such that $\|\xi_k-\1(\tilde{\alpha}_k+a_k)\|\to 0$, letting $\alpha_k=\tilde{\alpha}_k+a_k$ concludes the induction step. By the equivalence of consensus it follows that $x$ achieves $n$\ts{th}-order consensus.
% \end{proof}

So the previous theorem asserts that consensus will be achieved, now, we will focus on scalable performance. In this case we are interested in providing guarantees on worst-case transient behavior and is related to the behavior of weakly contracting systems.

Here follows a motivating example of

\begin{example}
    Consider $\dot{x}_i=-\mathrm{dz}\left(\sum_{k\in \mathcal{N}_i} x_i-x_k\right)$,
    obviously, this system is not guaranteed to achieve consensus, since the agents are only considering the deadzone, however, we can still show that this system is weakly contracting in terms the norm $\|\cdot\|_\infty$. This follows by looking at the dynamics of the maximal and minimum elements:

    $$\dot{x}_\mathrm{max}=-\mathrm{dz}\left(\sum_{k\in \mathcal{N}_i} x_\mathrm{max}-x_k\right)\leq -\mathrm{dz}(0) $$
    and likewise, $x_\mathrm{min}\geq 0$, which together show that $D^+\|x\|_\infty \leq 0$, where $D^+$ is the Dini derivative. This imply that $\|x(t)\|_\infty\leq\|x(0)\|_\infty$ for all $t\geq 0$
\end{example}

Now, we want to generalize our results on scalable performance to potentially non-linear consensus protocols. To do this, we first establish the calculus of scalable performance, that is, what operations preserve scalable 

\begin{theorem}
    The following system
    \begin{equation}
        \left((\partial_t+F_n)\circ (\partial_t+F_{n-1})\circ \dots\circ(\partial_t+F_1)\right)(x,t)=u_\mathrm{ref}
        \label{eq:nonlinear_serial}
    \end{equation}
    will satisfy $\left(F_n\circ F_{n-1}\circ\dots\circ F_1\right)(x_2-x_1)\to 0$ for any two solutions $x_1,x_2$.
\end{theorem}
\vspace{.5ex}
\begin{proof}
        
\end{proof}



\subsection{Halanay Inequality}
Here we will utilize the Halanay inequality to prove that the closed-loop system will satisfy scalable performance. This is true, even when all agents are actuated asynchronously.

There is a generalized version of the Halanay inequality which applies in the following setting \cite{Mazenc2022Halanay}:
\begin{equation}
    \bmat{\dot v_1(t)\\ \vdots \\ \dot v_n(t)} 
    \leq M \bmat{ v_1(t)\\  \vdots \\ v_n(t)} +P\bmat{\underset{l\in[t-\tau]}{\sup} v_1(l)\\ \vdots \\\underset{l\in[t-\tau]}{\sup} v_n(l) }.
    \label{eq:halanay}
\end{equation}
Here, $M$ is Metzler and $P$ is a nonnegative matrix and $v_k:\,[-\tau,\infty)\to R_+$. 
The system \eqref{eq:halanay}, where the inequality is changed to an equaliy, is asymptotically stable if and only if $R+P$ is Hurwitz. This serves as a comparison function to prove stability for all systems satisfying the inequality.

To apply this useful result in the vehicle platooning setting, we can look into where potential delays may appear.
\begin{align*}
    \ddot{x}_i(t)&=u_i(y(t-\tau_1(t)))\\
    y_i(t)&=\bmat{L_ix(t)\\L_i Lx(t)\\ L_i\dot x(t)}
\end{align*}
One clear candidate is that of actuation delay. This is due to multiple reasons; 1) the measurements may need to be transmitted between neighbors; 2) the local controllers need to be discretized and thus work through a zero-order hold discretization.

\begin{example}[First-order consensus with delay]
    We consider the following system:
        $$\dot{x}_i=-L_ix(t-\tau)$$
    This system is apparently not on the form \eqref{eq:halanay}, but it can be made close.
    Consider the control law:
    $$u(x)=-M(x(t)-x(t-\tau))$$
\end{example}




 


\subsection{Characterizing all systems with scalable performance}
Here, we pose a reverse question: given weakly contracting functions, how can they be combined while preserving the weakly contraction property?

So what are we after? When constructing coordination protocols, the locality constraint is often mirrored in each feedback term. As an example, we have:

$$\xi =\bmat{0& I\\
            -L_1& -L_2}\xi+\bmat{0\\u_\mathrm{ref}}$$
Now comes the interesting part: since $L_1$ and $L_2$ both contain a zero-eigenvalue, the best we can hope for is that a linear transformation exists to a system that is weakly contracting.
$$\bmat{L_3& 0\\
        0 & L_4}T=T\bmat{0& I\\
            -L_1& -L_2}$$    
Let's start with the simplest case, $2\times 2$ and present the results in the induced $\ell_\infty$ norm. Any positive diagonally scaled version of a weakly contracting system will also be weakly contracting. Furthermore, any permutation will also preserve stability. To work for a general graph Laplacian $L$, we will only consider the cases with block transformations. This result in:

$$\bmat{L_1& 0\\
        0 & L_2
        }T=T\bmat{0& I\\
            -L_1& -L_2}$$  



==> articlefiles/oldfiles/MathPrels.tex <==
\section{Mathematical Preliminaries}\label{sec:mathprel}
\emma{make preliminaries subsection in introduction. Move section C serial consensus to make it an example in Problem setup. 
}

\subsection{Graph theory}
We denote a graph as $\mathcal{G}(\mathcal{V},\mathcal{E})$ with $N=|\mathcal{V}|$ vertices and $\mathcal{E}\subset \mathcal{V}\times \mathcal{V}$ edges. The graph can also be defined with the adjacency matrix $W$, where $W_{i,j}>0 \iff(j,i)\in \mathcal{E}.$ Associated with an adjacency matrix, the graph Laplacian can be constructed as 
$$L=D-W$$
where $D$ is a diagonal matrix with its $i$\ts{th} element defined as $D_{ii}=\sum_{j=1}^N W_{ij}$. 

A graph is said to contain a directed spanning tree if a node $k\in \mc{V}$ exists such that every other node $j \in \mc{V}\setminus k$ is reachable through a path originating from $k$. If a graph contains a directed spanning tree, then its graph Laplacian will have a unique zero eigenvalue, and all other eigenvalues will have strictly positive real parts. 

Throughout this article, we will use standard notation for norms. With $\|x\|_\infty=\max_i |x_i|$ when $x\in \mathbb{C}^N$ and we use the same notation for the corresponding induced matrix norm $\|C\|_\infty=\max_i \sum_j |C_{i,j}|$. Functions composition will be denoted $(f\circ g)(x)=f(g(x))$. 

\subsection{Consensus}

Central for this work is the concept of consensus. 
\begin{definition}[Consensus]\label{def:consensus}
    A dynamical system 
    $$\dot{x}=f(x,t)$$
    where $x\in \RN$ is said to achieve consensus if $\lim_{t\to\infty}|x_i(t)-x_j(t)|=0$ for all $i\neq j$.
\end{definition}
A typical linear system that achieves consensus is 
$$\dot{x}=-Lx,$$
where $L$ is a graph Laplacian where the corresponding underlying graph contains a spanning tree. 

Sometimes it is desirable to reach consensus in multiple states simultaneously, often, these are related derivatives, such as positions, velocities, and accelerations. Achieving this is called 
\begin{definition}[$n\ts{th}$-order consensus]
    A dynamical system 
    $$\dfrac{\mathrm{d}^nx}{\mathrm{d}t^n}=f(x,t)$$
    where $x(t)\in \RN$ is said to achieve an $n\ts{th}$-order consensus if $\lim_{t\to\infty}|x^{(k)}_i(t)-x^{(k)}_j(t)|=0$ for all $i\neq j$ and $k \in [0,1,\dots,n-1]$.
\end{definition}

\subsection{Serial consensus}
This work builds on the idea of serial consensus where the closed-loop system is designed to match the behavior of regular consensus protocols put in a series interconnection. The $n\ts{th}$-order serial consensus system can in the Laplace domain be represented as 
$$(sI+L_n)\cdots(sI+L_2)(sI+L_1)X(s)=U_\mathrm{ref}(s).$$
One property that makes this system interesting is the simple condition for stability, that is, if each of the graphs underlying the $L_k$'s contain a directed spanning tree, then this high-order consensus protocol will achieve a $n\ts{th}$-order consensus, given a decaying input signal $\|u_\mathrm{ref}(t)\|\to 0$ \cite{jour:hansson2023scalable}. The serial consensus protocol can also be used to construct linear time-invariant consensus protocols for vehicular formations that has a strong notion of scalable performance \cite{jour:hansson2025tcns ,jour:hansson2024lcss}. 

To implement serial consensus there may be a need for extra signaling in the multi-agent system. This can be seen in the second-order serial consensus where the control law is
$$u(x,t)= -(L_1+L_2)\dot{x}-L_2L_1x,$$
where the velocity feedback can be realized through local measurements and for the second term, each agent can first aid to calculate $e=L_1x$, and the message pass this measurement to their followers so that they can calculate the relative differences of $L_2 e$. In general, it's possible to calculate the local control law for the $n\ts{th}$-order serial consensus through the use of $n-1$ local message passes; the local consensus protocol is only dependent on relative measurements within an $n$-hop neighborhood of each agent.

==> articlefiles/oldfiles/Numerical.tex <==
\section{Numerical Examples}

Here we will discuss a few interesting examples of nonlinear second-order consensus and illustrate how they perform through simulations. Common for all of the following examples is that they are trying to coordinate a platoon consisting of $N$ double integrators
\begin{equation}
    \ddot{x}=u(x,t)
\end{equation}
with the goal to maintain a fixed inter-vehicle distance. The control law that will be tested are designed through second-order serial consensus, that is,
\begin{equation}
    u(x,t)=-\Lc_2(\dot{x}(t) +\Lc_1(x(t),t),t)-\dt(\Lc_1(x(t),t))
\end{equation}
Although the results hold true for any graph structure, for simplicity, a uni-directional line graph structure will be used here. The following graph Laplacian will be used in all of the examples
\begin{equation}
    \Las=\bmat{0& 0 \\ -1 & 1 \\  & \ddots& \ddots\\ & & -1& 1}
    \label{eq:Las}
\end{equation}
In this network structure, the first vehicle can be seen as a leader, either virtual or real. For the subsequent simulations, the leader will start driving at $10$~m/s, with the rest of the network starting at a stand-still.


\subsection{Example: time-varying weights}
In this first example, a linear but time-varying consensus protocol will be used, in particular, 
$$\Lc_1(x,t)=D_1(t)\Las (x-d),\; \Lc_2(x,t)=D_2(t)\Las x$$
where $D_1,D_2$ are bounded, time-varying, and piecewise continuous non-negative diagonal matrices. Let's first check that all assumptions for Theorem~\ref{thrm:nonlinear_serial} are satisfied. Assumption~\ref{ass:stab_cons} follows from \cite{Moreau2004stabconsensus} \textbf{check which theorem} which establishes exponential stability of the consensus equilibrium together with \cite{jour:khalil2002nonlinear}\textbf{chapter 4?} that assures BIBO stability of such systems. Assumption~\ref{ass:invariance} follows since $\Las \1 a(t)=0$, and Assumption~\ref{ass:existandunique} follows from the assumption on $D_1$ and $D_2$.  So when using two such operators, the resulting serial interconnection should be stable.
\begin{example} 
 Let $[D_1(t)]_{k,k}=\max\{\sin(\omega_k t +\phi_k),0\}$ and $=D_2(t)=D_1(t)$, where $\omega_k\neq0$ and $\phi_k\in[0,2\pi)$ and $d_2>0$. For this choice of $D_1, D_2$, all requirements are satisfied and the resulting closed-loop system will converge to a consensus as asserted per Theorem~\ref{thrm:nonlinear_serial}. A simulation of the system is shown in \figref{fig:timevaryinggraph}. As expected, the agent experience a transient before converging to the desired formation. It is noteworthy that each of the agents use no feedback for half of the time, but still achieve consensus since the time integrated consensus graph is connected for a sufficiently large time window.

 \begin{figure}
     \centering
     \includegraphics[width=1\linewidth]{Figures/timevaryinggraphplot.pdf}
     \caption{A simulation of a platoon, where the leader drives at a constant velocity while the followers use time-varying weights to coordinate.}
     \label{fig:timevaryinggraph}
 \end{figure}
\end{example}


\subsection{Example: saturated signals}

For this example a commonly present nonlinearity will be used, the saturation function. This can be incorporated in the control when there is an actuation constraint limiting the available control capability. In this case, the corresponding consensus operators will be 
$$\Lc_1(x,t)=\mathrm{sat}\left( \Las(x-d)\right),\;\Lc_2(x,t)=\mathrm{sat}\left( \Las x\right),$$ 
where $\mathrm{sat}(\cdot)$ is the element-wise saturation function. In this case, Assumptions~\ref{ass:invariance},~\ref{ass:existandunique} are easy to verify for $\Lc_1$ and $\Lc_2$. That $\Lc_1$ is locally input-output stable is more involved \textbf{include proof here?}, but is possible to show. Thus, using these operators will also lead to a system with a stable consensus equilibrium. The result of a simulation is shown in \figref{fig:saturationplot}. The agents reach the desired formation


 \begin{figure}
     \centering
     \includegraphics[width=1\linewidth]{Figures/saturationlapplot.pdf}
     \caption{A simulation of a platoon, where the leader drives at a constant velocity while the followers use a serial consensus protocol with saturated signals. The agents experience two phases, first they coordinate in velocity and then some final positional adjustments are made to reach the desired formation.}
     \label{fig:saturationplot}
 \end{figure}


% \begin{example}
%     In a natural vehicle formation, one behavior that the drivers may exhibit is a periodic feedback, that is, the drivers routinely observe their neighborhoods and adjust based on this to then pause before repeating its coordination. One such system is the following
%     $$ \dot{x}$$
% \end{example}

\subsection{Example: actuation delays}
The regular linear serial consensus protocol uses the control law
$$u(x,t)=-(p_2+p_1)L\dot{x}-p_2p_1L^2x.$$
To implement this in a physical system, it might be necessary that the agents communicate and share signals, as is discussed in \cite{jour:hansson2025tcns}. Such process might introduce delays in the passed measurements. The following example illustrate that with a simple modification, this problem can be handled through serial consensus.
\begin{example}
    Let $[\mathcal{W}_\tau(x,t)]_i=\sum_{j\in \Nc_i} w_{i,j}(t)x(t-\tau_{i,j}(t))$ be the $i\ts{th}$ component of the vector $\mathcal{W}_\tau(x)$ and let $D_{i,i}(t)=\sum_{j\in \Nc_i} w_{i,j}(t)$ be a nonnegative diagonal matrix. The consensus protocol
    $$\dot{x}=-D(t)x(t)+\mathcal{W}_\tau(x(t),t)$$
    will have exponential convergence to a consensus, given sufficient connectivity and that there exists an upper bound on the local delay functions $\tau_{i,j}(t)\leq \tau_\mathrm{max}<\infty$ that holds for all $t\geq 0$. This is sufficient to use this consensus protocol for $\Lc_2$. However this consensus protocol is not guaranteed to achieve consensus when used for $\Lc_1$, because this operator does not satisfy Assumption~\ref{ass:invariance}. An example of what happens is found in Appendix~\ref{app:counterexample}. Now, the closed-loop system be given by
    \begin{equation}
        \left((\dt+D-\mathcal{W}_\tau)\circ (\dt +L)\right)(x)=0
    \end{equation}
    with the corresponding controller
    \begin{equation}
        u(x,t)= -L\dot{x}-(D\dot{x}-\mathcal{W}_\tau(\dot{x}))-DLx-\mathcal{W}_\tau(Lx).
    \end{equation}
    This controller deserves some explaining and discussion on implementation. The terms $L\dot{x}$ and $DLx$ are simply relative feedback with respect to each agents' neighbors. The term $\mathcal{W}_\tau(e)$, where $e=Lx$ are the delayed message passed relative measurements. The $i\ts{th}$ agent would use the following 
    $$[\mathcal{W}_\tau(e)]_i=\sum_{j\in\Nc_i} w_{i,j}e_i(t-\tau_{i,j}(t)).$$
    The final two terms $D\dot{x}-\mathcal{W}_\tau(\dot{x})$ are not necessarily locally measureable. However it can also be realized in the following way
    \begin{align*}
        &[D\dot{x}-\mathcal{W}_\tau(\dot{x})]_i=\sum_{j\in\Nc_i} w_{i,j}(\dot{x}_i(t)-\dot{x}_{j}(t-\tau_{i,j})\\
        & =\!\! \sum_{j\in\Nc_i} \!\!w_{i,j}\!\left( \dot{x}_i(t)-\dot{x}_{i}(t-\tau_{i,j})\!+\!\dot{x}_{i}(t-\tau_{i,j})-\dot{x}_{j}(t-\tau_{i,j})\right)
    \end{align*}
    The first two terms $\dot{x}_i(t)-\dot{x}_i(t-\tau_{i,j}(t))$ correspond to the change of velocity from $t-\tau_{i,j}(t)$ to the current time $t$ and can be tracked with onboard velocity sensors. The second pair $\dot{x}_i(t-\tau_{i,j}(t))-\dot{x}_j(t-\tau_{i,j}(t))$ is a delayed relative velocity measurement, and given the capability of measuring relative velocities, with some additional memory this signal can also be measured locally and then be synchronized with the delayed and message passed relative position measurement.

    A simulation, using the outlined consensus protocol with delayed measurements, is shown in \figref{fig:delayneighb}.


     \begin{figure}
     \centering
     \includegraphics[width=1\linewidth]{Figures/delayneighbplot.pdf}
     \caption{A simulation of a platoon, where the leader drives at a constant velocity while the followers use a serial consensus protocol with delayed and message passed measurements from their neighbors. The relative measurements are sampled through a Poisson distribution with average sample time of $2$~s. After a short transient the agents eventually reach the desired formation. }
     \label{fig:delayneighb}
 \end{figure}
   
    % [D\dot{x}-\mathcal{W}_\tau(\dot{x})]_i=\sum_{j\in\Nc_i} w_{i,j}(\dot{x}_i(t)-\dot{x}_{i}(t-\tau_{i,j}(t))+\dot{x}_{i}(t-\tau_{i,j}(t))-\dot{x}_{j}(t-\tau_{i,j}(t))$$
\end{example}


\subsection{Example: delayed GPS measurements}
% \begin{example}
%     Consider a vehicle formation consisting of $N$ double integrator systems
%     $$\ddot{x}=u(x,t).$$
%     The agents have access to local relative measurements in the platoon and a delayed and sampled GPS-based measurements of their absolute position. A first-order consensus protocol that utilize this additional information is
%     $$\dot{x}=-Lx-PS_\tau(x(t)-\1 x_0(t)+\ur=-\Lc(x,t)+\ur$$
%     Using 
% \end{example}
A similar example to the previous is when GPS signals are used for platooning. Like in the previous case, a delayed measurement can be used to coordinate with the leading vehicle. In this case the corresponding first-order system is
$$\dot{x}_i=-\underset{[\Lc_2(x,t)]_i}{\underbrace{P_{i,i}(x_i-x_1(t-\tau_i(t)))}}.$$
Using a regular linear consensus protocol $\Lc_1(x,t)=Lx$ results in the following closed-loop system
\begin{equation}
    \ddot{x}_i=-P_{i,i}(\dot{x}_i-\dot{x}_1(t-\tau_i(t))-\dot{e}_i-P_{i,i}(e_i-e_1(t-\tau(t))
\end{equation}
Once again, some discussion is warranted. In a leader-follower network, the perceived error of the leading vehicle is $e_1=0$, which follow from the first row being all zeros, see e.g. $\Las$ in \eqref{eq:Las}. $P_{i,i}e_i$ and $\dot{e}_i$ are scaled versions of the locally perceived relative error and relative velocity. For the first term, it is possible that there is a bias between the GPS and local velocity sensor, so here the trick of adding and subtracting to instead consider 
$$-P_{i,i}\left((\dot{x}_i -\dot{x}_i(t-\tau_i(t)))-(\dot{x}_1(t-\tau_i(t))-\dot{x}_i(t-\tau_i(t))\right),$$
which consist of a comparison of current velocity to a previous, and a delayed relative velocity measurement of vehicle deviation from the target velocity. 

A simulation of a platoon using delayed GPS measurements is presented in \figref{fig:delayneighb}. This consensus protocol can use the absolute feedback to quickly reject the velocity errors with the least transient error of all the presented protocols. 

 \begin{figure}
     \centering
     \includegraphics[width=1\linewidth]{Figures/delaygps.pdf}
     \caption{A simulation of a platoon, where the leader drives at a constant velocity while the followers use a serial consensus protocol with delayed relative velocity measurements to the leading vehicle. The delayed relative velocity measurements are sampled through a Poisson distribution with average sample time of $2$~s. After a short transient the agents eventually reach the desired formation.  }
     \label{fig:delayneighb}
 \end{figure}





% \begin{figure}
%     \centering
%     \begin{subfigure}[]{.48\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{Figures/hill_positions.pdf}
%         \caption{Position for all vehicles, using PI controller. }
%         \label{fig:3order_hill_pos}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[]{.48\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{Figures/2order_hill_positions.pdf}
%         \caption{Position for all vehicles, using proportional controller.}
%         \label{fig:secondorder_hill_pos}
%     \end{subfigure}
%    \medskip
%     \begin{subfigure}[]{.48\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{Figures/hill_relerror.pdf}
%         \caption{Deviation from desired relative position for all vehicles, using PI controller.}
%         \label{fig:3order_hill_rel}
%     \end{subfigure} 
%     \hfill
%         \begin{subfigure}[]{.48\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{Figures/2order_hill_relerror.pdf}
%         \caption{Deviation from desired relative position for all vehicles, using Proportional controller controller.}
%         \label{fig:secondorder_hill_rel}
%     \end{subfigure} 
%     \caption{Simulation of $40$ agents driving uphill at an inclination ratio $\theta=0.1$, and with a leader velocity $10$ m/s. The agents that use a serial consensus-based PI controller experience a transient and then return to the desired spacing. The vehicles controlled with a proportional controller experience a transient before settling with stationary error.}
%     \label{fig:3order_hill}
% \end{figure}

% \end{example}

==> articlefiles/oldfiles/Preliminaries.tex <==
\subsection{Definitions and network model}
We will by $\mc G(\mc V,\mc E)$ denote a graph with $N=|\mc V|$ vertices and with edge set $\mc E\subset \mc V\times \mc V$. 
The graph can also be represented by the weighted adjacency matrix $W$, which satisfies $w_{ij}>0 \iff (j, i)\in \mc V$. The graph is called undirected if $W^T=W$. The graph Laplacian $L$ is defined as $L=D-W$ where $D=\mathrm{diag}(W\mathbf{1})$.

A graph contains a directed spanning tree if, for some node $i$, a path exists to all other vertices $j\in \mc V \setminus i$. If the graph contains a directed spanning tree, then the associated graph Laplacian has a unique zero eigenvalue, and the rest of the eigenvalues have strictly positive real parts.

Throughout this paper we will denote the standard vector $\infty$-norm of $x\in \mathbb C^N$ as $\|x\|_\infty=\max_i |x_i|$. We will reuse the notation for the corresponding induced matrix norm of $C\in \mathbb C^{M\times N} $, that is, $\|C\|_\infty=\sup_{\|x\|_\infty=1} \|C x\|_\infty=\max_i \sum_{j=1}^N |C_{ij}|$. We denote the standard Kronecker product between two matrices  $A\otimes B$.

\subsection{Serial Consensus}
% Serial consensus, what to include? 
% 
We begin by introducing serial consensus.
\begin{definition}[$n\ts{th}$-order serial consensus]
    The following closed-loop system, expressed in the Laplace domain,
    \begin{equation}
        \left(\prod_{k=1}^n sI+L_k\right)X(s)=U_\mathrm{ref}(s)
        \label{eq:def_serial_consensus}
    \end{equation}
    is called the $n\ts{th}$-order serial consensus system.
\end{definition}
This can be compared to the conventional $n\ts{th}$-order consensus system which in the case $n=2$ would be
$$\ddot{x}=-L_1\dot{x}(t)-L_0x(t)+u_\mathrm{ref}(t).$$
The corresponding second-order serial consensus system is
$$\ddot{x}(t)=-(L_2+L_1)\dot{x}-L_2L_1x+u_\mathrm{ref}.$$
The two protocols are similar and can be seen as two natural ways of generalizing the regular continuous-time consensus protocol, that is, $\dot x=-Lx$, preserving the limitation of only utilizing relative feedback. We refer to \cite{Hansson2023CDC} for a more elaborate discussion.

One practical property of the serial consensus is that there exists a simple sufficient condition for stability; under the assumption that each of the graph Laplacians $L_k$ each contains a directed spanning tree, the serial consensus is known to eventually achieve coordination \cite{Hansson2023CDC}. When the same graph Laplacians are used, i.e., $L_k=p_kL$, then some additional performance results can be proven, which will be studied later in this paper. In this case, the serial consensus system can be represented in the following state-space form
$$
    \bmat{\dot x\\ \ddot x\\\vdots\\x^{(n)}}
\hspace{-.5ex}\!=\!\hspace{-.5ex}\bmat{ & \hspace{-2ex}I \\
       &  & \hspace{-2ex}\ddots\\
       &  &  &\hspace{-2ex} I\\
       -a_0L^n&\hspace{-1.5ex}- a_1L^{n-1}& \hspace{-2ex}\dots &\hspace{-1.5ex}-a_{n-1}L }
       \hspace{-.9ex}\bmat{ x\\ \dot x\\ \vdots\\x^{(n-1)}}\hspace{-.6ex}+\hspace{-.6ex}
       \bmat{\\ \\ \\u_\mathrm{ref}}\!\!,
$$
where $a_k$ are identified with the weights $p_k$ through the relation $\prod_{k=1}^n(s+p_k)=\sum_{k=0}^{n} a_ks^k$.
Another state space representation that will be of interest is given by
\begin{equation}
    \underbrace{\bmat{ L^{n-1}\dot x\\  L^{n-2}\ddot x\\\vdots\\x^{(n)}}}_{\dot{\xi}}
\hspace{-.65ex}=\hspace{-.65ex}\underbrace{\bmat{ & \hspace{-2ex}L \\
       &  & \hspace{-2ex}\ddots\\
       &  &  &\hspace{-2ex} L\\
       -a_0L&\hspace{-1.5ex}- a_1L& \hspace{-1ex}\dots &\hspace{-2.ex}-a_{n-1}L }}_{\mc A=A\otimes L}
       \hspace{-.5ex}\underbrace{\bmat{ L^{n-1}x\\ L^{n-2}\dot{x}\\ \vdots\\x^{(n-1)}}}_\xi\hspace{-.5ex}+\hspace{-.5ex}
       \bmat{\\ \\ \\u_\mathrm{ref}}\!\!,
       \label{eq:xistates}
\end{equation}
where 
\begin{equation}\label{eq:A}
    A=\bmat{& 1 \\
          & & \ddots\\
            & & & 1\\
            -a_0&-a_1 &\dots &-a_{n-1}}.
\end{equation}
Here, we note that $A$ is in the controllable canonical form associated with the transfer function
$\prod_{k=1}^n(s+p_k)^{-1}.$





\subsection{Scalable performance}

The performance of a system can be evaluated in multiple ways. Inspired by the setting of vehicle formations where velocity following and relative distance keeping is required, we define the measurements $e_\mathrm{pos}=L(x-d)$ and $e_\mathrm{vel}=\dot{x}-v_\mathrm{ref}\mathbf{1}$ with $d\in\mathbb{R}^n$ and $v_\mathrm{ref}\in \mathbb R$ to be the quantities that should be kept small throughout the dynamic phase. This leads to the following definition.
\begin{definition}[Scalable Performance]
    A formation controller defined over a growing family of graphs $\{\mathcal G_N\}$ that ensures 
\begin{equation}
    \sup_{t\geq 0} \left\|\bmat{e_p(t)\\e_v(t)}\right\|_\infty \leq \alpha \left\|\bmat{e_p(0)\\e_v(0)}\right\|_\infty,
    \label{eq:scalable_performance}
\end{equation}
where $\alpha$ is fixed and independent of the number of agents $N$, is said to achieve scalable performance.  
\end{definition}
\vspace{.5ex}
The choice of the norm here is important since the maximum deviations from an equilibrium determine whether collisions will occur or speed limits will be violated.

This definition cannot be directly applied to a more general system since performance is application-dependent. Instead, we consider a more general definition for the high-order consensus protocols.
\begin{definition}[Scalable $\mathcal{C}$-performance]
    A formation controller for the system $\dot{\xi}=-\mc A\xi+\mc B w$ with $y=\mc C \xi$ defined over a growing family of graphs $\{\mathcal G_N\}$ that ensures 
    $$\sup_{t\geq0}  \|y\|_\infty \leq \alpha_y\|y(0)\|_\infty +\alpha_w\sup_{t\geq0}\|w\|_\infty, $$
    where $\alpha_y,\alpha_w$ are fixed and independent of the number of agents $N$, is said to achieve scalable $\mathcal{C}$-performance. 
\end{definition}
We note that this definition is close to scalable input-to-state stability \cite{Besselink2018}. However, here we omit the restriction of having a convergence rate independent of the number of agents. In the case of vehicle formations, and using the measurements $e_\mathrm{pos}$ and $e_\mathrm{vel}$, scalable $\mathcal{C}$-performance implies that no vehicle will deviate far from the desired formation and desired velocity at any point in time. These, we argue, are the main objectives in this setting, while a uniform convergence rate is secondary and potentially not even feasible due to locality and gain constraints.

==> articlefiles/oldfiles/mainResultsnew.tex <==
\section{Main Results}
\emma{Completely restructure as agreed. In the proof, first explain the steps that you take. Then include the lemmas (now theorems). Their proofs in turn can be sketched, but main proofs moved to appendix.  }






\begin{theorem}\label{thrm:consensusequivalnce}
    $\Lc_k$ satisfy Assumption~\ref{ass:kiscont} for all $0 \leq k+j\leq n-1$, and all time $t$. Then, the following two are equivalent:
\begin{itemize}
    \item[i)] The solution $x$ of the compositional consensus \eqref{eq:nonlinear_serial} achieves $n\ts{th}$-order consensus for any initial condition;
    \item[ii)] the states $\xi_k$ where $k=1,...,n$ of \eqref{eq:statespace} achieves first-order consensus for any initial condition.
\end{itemize}
\end{theorem}
\emma{Introduce function B before Lemma?} To prove this result, we will use the following Lemma.
\begin{lemma}\label{lem:consensus_invariance}
    Let $\Lc\in \C^n$ and satisfy $\Lc(z+\1 a(t),t)$ for any integrable function $a(t)$, then, for any $k\leq n$ the following is true: $\dtk{k}\Lc(z,t)=B_k(z,\dot{z},\dots,z^{(k)},t)=B_k(z-\1 b_0(t),\dot{z}-\1 b_1(t),\dots,z^{(k)}-\1 b_k(t),t)$ for any integrable functions $b_1, b_2,\dots, b_k$.
\end{lemma}
\begin{proof}
    We prove this by induction. The base case is directly proven by $B_0(x)=\Lc(x,t)$. Now, suppose it is valid for $k\leq n-1$. Firstly, taking the partial derivatives for any $ j \leq k$: $\partial_{z^{(j)}} B_k(z,\dots,z^{(k)},t)=\partial_{z^{(j)}} B_k(z-\1 b_0(t),\dots,x^{(k)}-\1 b_k(t),t)$. This shows that all partial derivatives are invariant to arbitrary translation along the consensus, and the same argument also holds for the partial time derivative. Now, taking the time derivative of the consensus translated  equation results in:
    \begin{multline*}
        \dtk{k+1}\Lc(x,t)=\partial_t B_k(x-\1 c_0(t),\dots,x^{(k)}-\1 c_k(t),t)+\\ \sum_{j=0}^k \!\partial_{x^{(j)}} B_k(x-\1 c_0(t),\dots,x^{(k)}-\1 c_k(t),t) (x^{(j+1)}-\1\dot{c}_j(t))
    \end{multline*}
Let $c_j(t)=\int_0^tb_{j+1}(\tau)\mathrm{d}\tau$ and for each partial derivative term do the outlined translation to get
\begin{multline*}
        \dtk{k+1}\Lc(x,t)=\partial_t B_k(x-\1 b_0(t),\dots,x^{(k)}-\1 b_k(t),t)+\\ \sum_{j=0}^k\! \partial_{x^{(j)}}\! B_k(x-\1 b_0(t), \!... ,x^{(k)}\!\!-\1 b_k(t),t) (x^{(j+1)}\!\!-\1 b_{j+1}(t)).
    \end{multline*}
    This shows the sought translation invariance and concludes the proof.
\end{proof}

Next, we prove the theorem.

\begin{proof}
    First, we establish that the initial condition of $\xi_k$ is uniquely determined by the initial condition $x$  and its first $n-1$ derivatives. By using the relation $x=\xi_1$ and \eqref{eq:statespace}, the following relation can be derived
    $$x^{(j)}=-\dtk{j-1}\Lc_1(\xi_1,t)-\dots-\Lc_j(\xi_j,t)+\xi_{j+1}.$$
    Due to the smoothness of $\Lc_k$, it is possible to expand the time derivatives in terms of the partial derivatives through the chain rule. The time derivatives can thus be expressed as
    $$\dtk{j}\Lc_k(\xi_k,t)=B_{k,j}(\xi_k,\dot{\xi}_k,\dots,\xi_k^{(j)},t).$$
    Since $\dot{\xi}_k=-\Lc_k(\xi_k,t)+\xi_{k+1}$, it is possible to reduce the derivative dependence recursively and to show that \emma{I felt I wanted a middle step here?}
    $$\dtk{j}\Lc_k(\xi_k,t)=\hat{B}_{k,j}(\xi_k,\xi_{k+1},\dots,\xi_{k+j},t).$$
    Applying this to the general case leads to 
    $$
        \xi_{j+1}=x^{(j)}+\sum_{k=1}^j \hat{B}_{k,j-k}(\xi_k,\dots,\xi_j,t), 
    $$
    \edit{ for $j = 0,\ldots,n-1$}.
    Evaluating this at $t=0$ shows that $\xi_{j+1}$ is uniquely determined by $x^{(j)}(0)$ and the initial conditions of $\xi_k(0)$ for $k\leq j$. This, together with $\xi_1(0)=x(0)$, can be used to prove that $\xi_k(0)$ is uniquely determined by the initial condition of $x$ and its derivatives through a simple induction hypothesis. A similar\emma{analogous?} proof can be made in the reverse direction and, therefore, is omitted.

    For the second part of the proof, we will show that consensus of the states $\xi_k$ implies that $x$ achieves $n\ts{th}$-order consensus. As induction hypothesis, assume that $\|\xi_k^{(j)}-\1 a_{k+j}(t)\|\to 0$, with the induction step taken in the $j$ direction. The base case follows from the assumption that $\xi_k$ all reach a consensus, that is $\|\xi_k-\1 a_k(t) \|\to 0$.

    For the induction step consider the general expression for $\xi_k^{(j+1)}$ for $k+j\leq n-1$, which is
$$\xi_k^{(j+1)}=-\dtk{j}\Lc_k(\xi_k,t)+\dtk{j}\xi_{k+1}.$$
Using Lemma~\ref{lem:consensus_invariance}, this can be expressed in terms of the translated states
    $$\xi_k^{(j+1)}=-B_{k,j}(\xi_k-\1 a_k(t),\dots,\xi_k^{(j)}-\1 a_{k+j},t)+\xi_{k+1}^{(j)}.$$
    By the premise of the theorem, $\|B_{k,j}\|$ can be bounded by $\alpha_{k,j}\in \mathcal{K}$. Subtracting $\1 a_{k+j+1}$ on both sides, taking the norm, using the triangle inequality, and bounding using the class $\mathcal{K}$ function $\alpha_{k,j}$ leads to
\begin{multline*}
    \|\xi_k^{(j+1)}-\1 a_{k+j+1}\|\leq \|\xi_{k+1}^{(j)}-\1 a_{k+j+1}(t)\| +\\\alpha_{k,j}\left(\max\left\{\|\xi_k-\1 a_k(t)\|,\dots,\|\xi_k^{(j)}-\1 a_{k+j}\|\right\}\right)
    \end{multline*} 
    Now, taking the limits on both sides, using the induction hypothesis together with the continuity of $\alpha_{k,j}$ shows that $\lim_{t\to \infty}\|\xi_k^{(j+1)}-\1 a_{k+j+1}(t)\|=0$. Thus $\xi_k$ achieves an $(n-k+1)$\ts{th}-order consensus. Since $x(t)=\xi_1$ it follows that $x$ achieves an $n$\ts{th}-order consensus.

    The other direction, that is, x achieving $n\ts{th}$ order consensus implying that $\xi_k$ achieves consensus is conducted similarly. Now, the induction hypothesis is that $\xi_{k}^{(j)}-\1 a_{j+k}(t)$ where this will be proved by induction steps in $k$.
    First, using the relation of $x(t)=\xi_1(t)$ shows that $\xi_1$ achieves $n$\ts{th} order consensus. The $n$\ts{th} order consensus implies that $\|\xi^{(j)}-\1 a_j(t)\| \to 0$ for some functions $a_j(t)$. For the induction step, we consider the relation
$$\dot{\xi}_k=-\Lc_k(\xi_k,t) +\xi_{k+1}$$
This can be derivated $j\leq n-k-1$ times, and be rearranged to
$$\xi_{k+1}^{(j)}-\1 a_{j+k+1}=\xi^{(j+1)}_k-\1 a_{j+k+1}+\dtk{j}\Lc_k(\xi_k,t).$$
Now, Lemma~\ref{lem:consensus_invariance} is used to express $\dtk{j} \Lc_k$ in terms of $B_{k,j}$ and in particular in the translated states 
$$ \dtk{j} \Lc_k(\xi_k,t)=B_{k,j}(\xi_k-\1 a_k(t),\dots,\xi_k^{(j)}(t)-\1 a_{k+j}(t),t). $$
Applying the triangle inequality, bounding $\|B_{k,j}\|$ with $\alpha_{k,j}$, and concluding by taking the limit shows that
$$\lim_{t\to \infty}\|\xi_{k+1}^{(j)}-\1 a_{j+k+1}\|=0$$
This proves the induction step. Since this also shows that $\|\xi_{k}-\1 a_k(t)\| \to 0$, we can conclude that the states will achieve consensus.
\end{proof}

With the equivalence between \eqref{eq:nonlinear_serial} and \eqref{eq:statespace}, our next step is to prove that the latter will achieve consensus under relatively mild conditions.
\begin{theorem}\label{thrm:statespaceconsensus}
    Suppose that $\Lc_n$ satisfies Assumption~\ref{ass:Ln_stable} and $\Lc_k(z,t)$ satisfy Assumption~\ref{ass:kislipschitz}--\ref{ass:kislocallyISS} for $k\neq n$, then all $\xi_k$ in \eqref{eq:statespace} will have a unique solution that satisfy
    $$\lim_{t\to \infty} \|\xi_k(t)-\1 a_k(t)=0$$
    for some functions $a_k(t)$.
\end{theorem}

\begin{proof}
    Existence and uniqueness of $\xi_n$ is part of Assumption~\ref{ass:Ln_stable}. For the remaining states it is simple to verify that Assumption~\ref{ass:kislipschitz} implies that \eqref{eq:statespace} is globally Lipschitz in $\xi_k$ and piecewise continuous in $t$. Existence and uniqueness follow from a standard application of Carathéodory's existence and uniqueness theorem.

    Through induction, we'll prove that consensus will be reached, that is $\|\xi_k-\1a_k(t)\|\to 0$ for some functions $a_k(\cdot)$. The base case with $\|\xi_n-\1 a_n(t)\|\to 0$ follows from our assumption. Suppose it is true for all $\xi_k$ where $k\geq p+1$. The solution for $\xi_p$ satisfy
$$\dot{\xi}_p(t)=-\Lc_p(\xi_p(t),t)+\xi_{p+1}(t)$$
Now, subtracting the asymptotic solution of $\xi_{p+1}$ from both sides and using the fundamental theorem of calculus results in
\begin{multline*}
    \dtk{}\left(\xi_p(t)-\1\int_0^t a_{p+1}(\tau)\mathrm{d}\tau\right)\\=-\Lc_p\left(\xi_p(t)-\1\int_0^t a_{p+1}(\tau)\mathrm{d}\tau,t\right)+\xi_{p+1}-\1 a_{p+1}(t),
    \end{multline*}

where the invariance of $\Lc_p$ through Assumption~\ref{ass:kisinvariant} was also used. Let $z_p(t)=\xi_p(t)-\1\int_0^t a_{p+1}(\tau)\mathrm{d}\tau$ and $w_p(t)=\xi_{p+1}-\1 a_{p+1}(t)$. Then  $z_p$ satisfies
$$\dot{z}_p=-\Lc_p(z_p,t)+w_p(t)$$
where $\|w_p(t)\|\to 0$, which allows us to apply Assumption~\ref{ass:kislocallyISS}. In particular, there is a time $T_p$ such that $\|w_p(t)\|\leq M_p$, where this system is ISS for some seminorm $\vertiii{\cdot}$. To assert that $\lim_{t\to \infty} \|z_p(t)-\1 b_p(t)\|=0$ we can use the $\epsilon$ and $T$ definition for the limit. For any $\epsilon>0$, choose $T_p'$ such that $\|w_p(t)\|<\gamma_k^{-1}(\epsilon/2)$ for all $t> T_p'$. Now, using the ISS property starting at $T_p'$, we get
$$\vertiii{z_p(t)}< \beta_p(\vertiii{z_p(T_p')},t)+\frac{\epsilon}{2}$$
By the definition of $\beta_p$ it's possible to choose a time $T\geq T_p'$ such that $\beta_p(\vertiii{z_p(T_p')},t)<\epsilon/2$.
This proves that the seminorm converges and in particular that there exists a $b_p(t)$ such that $\|z_p(t)-\1 b_p(t)\|\to 0\implies \|\xi_p(t)-\1\left(b_p(t)+\int_0^t a_{p+1}(\tau)\mathrm{d}\tau\right)\|\to 0$, letting $a_p=b_p(t)+\int_0^t a_{p+1}(\tau)\mathrm{d}\tau$ conclcudes the induction step.
\end{proof}

As a final result, we summarize the consequence for the compositional consensus system \eqref{eq:nonlinear_serial}. 
\begin{theorem}\label{thrm:asymptoticconsensus}
\emma{Rewrite as agreed: ``Let all $\mathcal{L}_k$ be subject to Assumption-relative- and achieve consensus individually in the sense that... $\lim_t\rightarrow\infty ||z-1s(t)||\rightarrow 0$. Additionaly let $\mathcal{L}_k$ , $k = 1,...,n-1$ satisfy Assumptions... . Then,....}
    If $\Lc_n$ satisfies Assumption~\ref{ass:Ln_stable} and for $k\neq n$ the operators $\Lc_k$ satisfy Assumptions~\ref{ass:kislipschitz}--\ref{ass:kiscont}. Then, the compositional consensus \eqref{eq:nonlinear_serial} has a unique solution $x$, which will achieve $n\ts{th}$-order consensus.
\end{theorem}
\begin{proof}
    The results follow from Theorems~\ref{thrm:consensusequivalnce} and \ref{thrm:statespaceconsensus}.
\end{proof} 

\emma{Make a new subsetion on implementation. There, you talk about the LTI case (some repetition from previous papers) but also about this assumption. What do we need from the $\mathcal{L}$s so that the $u$s can be computed?}
\begin{rem}
    The existence and uniqueness of the solution $x$ should be interpreted as a weak solution, which satisfies the original differential equation \eqref{eq:nonlinear_serial} almost everywhere. For the solution to be smooth and satisfy the original differential equation everywhere, one may assume $\Lc_k\in C^{n-k}$.
\end{rem}
\begin{conjecture}\label{conj:functionaldiff}
    The results of Theorem~\ref{thrm:asymptoticconsensus} applies to the class of functional differential equations, where smoothness is understood through the existence of Fréchet derivatives.
\end{conjecture}
This class includes differential equations of the type $\dot{x}=-\Lc(x_t,t)$, where for some $r\geq 0$, $A\geq 0$ and $\sigma\in \R$ we have $x\in C([-\sigma-r,\sigma+A],\R^N)$, and define $x_t(\theta)=x(t-\theta)$, where $0\leq \theta\leq r$. In particular, this class includes the class of time-delayed differential equations, like
\begin{equation}\label{eq:delay}
    \dot{x}=-\Lc(x(t-\tau_1(t)),\dots, x(t-\tau_p(t)),t),
\end{equation}
where $\tau_k(t)\leq r$. For reference on this topic we refer to \cite{jour:hale2013introductionfunctional}. 


% \begin{rem}
%     The results of Theorem~\ref{thrm:asymptoticconsensus} can be extended to the larger class of functional differential equations of the type $\dot{x}=-\Lc(x_t,t)$, where for some $r\geq 0$, $A\geq 0$ and $\sigma\in \R$ we have $x\in C([-\sigma-r,\sigma+A],\R^N)$, and define $x_t(\theta)=x(t-\theta)$, where $0\leq \theta\leq r$. In particular, this class includes the class of time-delayed differential equations, like
%     \begin{equation}\label{eq:delay}
%         \dot{x}=-\Lc(x(t-\tau_1(t)),\dots, x(t-\tau_p(t)),t),
%     \end{equation}
%     where $\tau_k(t)\leq r$. For reference on this topic we refer to \cite{jour:hale2013introductionfunctional}. 
% \end{rem}


\textbf{Jonas, for this first submission we might want to increase the differentiability order by 1 to really guarantee implementability of the controller, however, this would reduce the number of applications.}
